Scheduling Mechanisms in Wireless Sensor-Actuator Networks for Multi-rate Periodic Control in Industry 4.0

This paper investigates scheduling strategies for wireless sensor-actuator networks (WSANs) in Industry 4.0 scenarios. In particular, we address the problem of real-time scheduling for multi-rate control systems by proposing a novel framework. Our framework features four strategies that improve reliability, schedulability and execution time, and reduce communication and storage costs. Two-phase scheduling is our first strategy, devised to improve communication reliability. Our second strategy is the least-laxity-first with remaining conflicts (LLF-RC) scheduling algorithm, which has high schedulability and affordable execution time. LLF-RC also keeps the maximum queue length at a moderate level, making it suitable for storage-constrained devices. Our third and fourth strategies are opportunistic aggregation and repetitive scheduling. Opportunistic aggregation performs simple and effective packet aggregation, enhancing schedulability by up to 97% and reducing execution time by up to 29%, in our simulation. Repetitive scheduling has negligible execution time, and contributes to minimize communication and storage costs. It reduces the maximum execution time by 92% and the maximum communication and storage cost by 99%, in our simulation. We compare our proposed framework against existing approaches, and evaluate the advantages of our strategies in realistic scenarios.

==> preamble/title-authors.tex <==
% !TeX root = ../main.tex

\title{\huge Scheduling Mechanisms in Wireless Sensor-Actuator Networks \\ for Multi-rate Periodic Control in Industry 4.0}

\author{
\IEEEauthorblockN{Dingwen Yuan, 
				  Luis F. Abanto-Leon, and 
				  Matthias Hollick} \\ 
\IEEEauthorblockA{Secure Mobile Networking Lab, Technical University of Darmstadt, Germany \\
\normalsize pdvyuan@gmail.com, \{labanto, mhollick\}@seemoo.tu-darmstadt.de} 
}
